Backtranslation Feedback Improves User Confidence in MT, Not Quality

Translating text into a language unknown to the text's author, dubbed outbound translation, is a modern need for which the user experience has significant room for improvement, beyond the basic machine translation facility. We demonstrate this by showing three ways in which user confidence in the outbound translation, as well as its overall final quality, can be affected: backward translation, quality estimation (with alignment) and source paraphrasing. In this paper, we describe an experiment on outbound translation from English to Czech and Estonian. We examine the effects of each proposed feedback module and further focus on how the quality of machine translation systems influence these findings and the user perception of success. We show that backward translation feedback has a mixed effect on the whole process: it increases user confidence in the produced translation, but not the objective quality.

==> Makefile <==
LATEX=pdflatex
MAINFILE=MAIN


#$(MAINFILE).pdf: biblio.bib

pdf:
	$(LATEX) $(MAINFILE).tex
	$(LATEX) $(MAINFILE).tex
	$(LATEX) $(MAINFILE).tex
	bibtex $(MAINFILE) || ( echo "Bibtex failed" && exit 1 )
	$(LATEX) $(MAINFILE).tex
	$(LATEX) $(MAINFILE).tex
	$(LATEX) $(MAINFILE).tex
	#lim=4; \
	#  while [ $$lim -ge 0 ] \
	#      && grep 'Rerun to get\|Citation.*undefined' $*.log >/dev/null 2>/dev/null; do \
	#    $(LATEX) $(MAINFILE).tex ; \
	#    lim=$$(($$lim - 1)) ; \
	#  done
	cp $(MAINFILE).pdf PREVIEW.pdf

.PHONY: ci
ci:
	# make sure git will remember my password
	git config credential.helper store
	# git pull push dance with possibly uncommited local modifications
	if git pull; then echo No changes to hide; else git stash; git pull; git stash apply; fi; git commit -am "make ci by $(USER)"; git push

clean:
	rm -f $(MAINFILE).log $(MAINFILE).aux $(MAINFILE).bbl $(MAINFILE).blg $(MAINFILE).toc $(MAINFILE).out $(MAINFILE).run.xml $(MAINFILE).bcf


==> src/collected_summary.tex <==

%%%%%%%%%%
%%%%%%%%%%
Czech 1 & 610 \\
Czech 2 & 643  \\
Czech 3 & 601 \\
Estonian & 632 \\ \midrule
BT QE PP & 313 \\
BT QE & 333 \\
BT PP & 311 \\
QE PP & 308 \\
BT & 316 \\
QE & 305 \\
PP & 311 \\
- & 289 \\
\midrule
Total & 2486 \\

%%%%%%%%%%
%%%%%%%%%%

==> src/gb_qe_results_original.tex <==
% For backup only, because I rounded it to two decimal places -VZ
    Accuracy    & 0.738     & 0.761     & 0.766     & 0.697 \\
    F1          & 0.834     & 0.854     & 0.865     & 0.805 \\
    F1-neg      & 0.372     & 0.347     & 0.142     & 0.319 \\
    F1-pos      & 0.834     & 0.853     & 0.865     & 0.805 \\
    F1-mult     & 0.311     & 0.296     & 0.123     & 0.257 \\
    MCC         & 0.280     & 0.281     & 0.117     & 0.237 \\

==> src/mts_effect.tex <==

%%%%%%%%%%
%%%%%%%%%%
Czech MT 1 & 3.61 & 3.61 \\
Czech MT 2 & 3.89  &  3.89 \\
Czech MT 3 & 3.85 & 3.85 \\
Estonian &   3.76  &  3.76 \\ \hline
BT QE PP & 3.95 & 0 \\
BT QE & 3.90 & 0 \\
BT PP & 4.20 & 0 \\
QE PP & 3.59 & 0 \\
BT & 4.18 & 0 \\
QE & 3.14 & 0 \\
PP & 3.90 & 0 \\
- & 3.31 & 0 \\
\hline
Total & 0 & 0 \\

%%%%%%%%%%
%%%%%%%%%%
